The Man Behind the Curtain: X-rays Drive the UV through NIR Variability in the 2013 AGN Outburst in NGC 2617

After the All-Sky Automated Survey for SuperNovae (ASAS-SN) discovered a significant brightening of the inner region of NGC 2617, we began a ~70 day photometric and spectroscopic monitoring campaign from the X-ray through near-infrared (NIR) wavelengths. We report that NGC 2617 went through a dramatic outburst, during which its X-ray flux increased by over an order of magnitude followed by an increase of its optical/ultraviolet (UV) continuum flux by almost an order of magnitude. NGC 2617, classified as a Seyfert 1.8 galaxy in 2003, is now a Seyfert 1 due to the appearance of broad optical emission lines and a continuum blue bump. Such "changing look Active Galactic Nuclei (AGN)" are rare and provide us with important insights about AGN physics. Based on the Hbeta line width and the radius-luminosity relation, we estimate the mass of central black hole to be (4 +/- 1) x 10^7 M_sun. When we cross-correlate the light curves, we find that the disk emission lags the X-rays, with the lag becoming longer as we move from the UV (2-3 days) to the NIR (6-9 days). Also, the NIR is more heavily temporally smoothed than the UV. This can largely be explained by a simple model of a thermally emitting thin disk around a black hole of the estimated mass that is illuminated by the observed, variable X-ray fluxes.

==> tabphot_long.tex <==
\begin{deluxetable}{lrcc}
\tablewidth{400pt}
\tablecaption{Photometric Observations}
\tablehead{
\colhead{JD} &
\colhead{} &
\colhead{Magnitude | X-Ray Flux} &
\colhead{Photon Index} \\ 
\colhead{($-$2,450,000)} &
\colhead{Band} &
\colhead{ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ | [$10^{-11}$ ergs/cm$^{2}$/s]}  &
\colhead{$\Gamma$}  }
\startdata
6413.430 & X-Ray$_\mathrm{swift}$ & [2.84(0.12)] & 1.69(0.10) \\ 
6414.760 & X-Ray$_\mathrm{swift}$ & [2.29(0.12)] & 1.72(0.11) \\ 
6415.194 & X-Ray$_\mathrm{swift}$ & [2.34(0.12)] & 1.66(0.11) \\ 
6416.296 & X-Ray$_\mathrm{swift}$ & [2.32(0.10)] & 1.55(0.10) \\ 
6417.069 & X-Ray$_\mathrm{swift}$ & [2.79(0.12)] & 1.73(0.09) \\ 
6419.104 & X-Ray$_\mathrm{swift}$ & [6.80(0.15)] & 1.78(0.04) \\ 
6420.542 & X-Ray$_\mathrm{swift}$ & [9.14(0.25)] & 1.86(0.04) \\ 
6421.340 & X-Ray$_\mathrm{swift}$ & [8.64(0.18)] & 1.86(0.04) \\ 
6422.944 & X-Ray$_\mathrm{swift}$ & [8.49(0.10)] & 1.93(0.04) \\ 
6423.750 & X-Ray$_\mathrm{swift}$ & [8.48(0.25)] & 1.84(0.06) \\ 
6424.305 & X-Ray$_\mathrm{swift}$ & [6.86(0.16)] & 1.78(0.06) \\ 
6425.750 & X-Ray$_\mathrm{swift}$ & [7.06(0.26)] & 1.83(0.06) \\ 
6427.479 & X-Ray$_\mathrm{swift}$ & [6.62(0.18)] & 1.69(0.15) \\ 
6430.953 & X-Ray$_\mathrm{swift}$ & [6.94(0.38)] & 1.81(0.06) \\ 
6431.125 & X-Ray$_\mathrm{swift}$ & [7.22(0.27)] & 1.79(0.11) \\ 
6432.781 & X-Ray$_\mathrm{swift}$ & [6.48(0.16)] & 1.85(0.10) \\ 
6433.792 & X-Ray$_\mathrm{swift}$ & [8.70(0.18)] & 1.89(0.05) \\ 
6434.719 & X-Ray$_\mathrm{swift}$ & [8.64(0.18)] & 1.84(0.06) \\ 
6435.573 & X-Ray$_\mathrm{swift}$ & [8.07(0.16)] & 1.95(0.06) \\ 
6436.439 & X-Ray$_\mathrm{swift}$ & [9.12(0.22)] & 1.88(0.06) \\ 
6437.427 & X-Ray$_\mathrm{swift}$ & [8.67(0.20)] & 1.80(0.06) \\ 
6438.844 & X-Ray$_\mathrm{swift}$ & [7.05(0.20)] & 1.85(0.06) \\ 
6439.580 & X-Ray$_\mathrm{swift}$ & [8.83(0.43)] & 1.73(0.08) \\ 
6440.565 & X-Ray$_\mathrm{swift}$ & [6.04(0.30)] & 1.77(0.10) \\ 
6441.516 & X-Ray$_\mathrm{swift}$ & [6.61(0.18)] & 1.71(0.08) \\ 
6442.903 & X-Ray$_\mathrm{swift}$ & [3.96(0.16)] & 1.78(0.06) \\ 
6443.840 & X-Ray$_\mathrm{swift}$ & [3.48(0.13)] & 1.79(0.08) \\ 
6444.840 & X-Ray$_\mathrm{swift}$ & [2.18(0.15)] & 1.65(0.12) \\ 
6445.520 & X-Ray$_\mathrm{swift}$ & [0.73(0.09)] & 1.66(0.14) \\ 
6447.042 & X-Ray$_\mathrm{swift}$ & [1.91(0.10)] & 1.74(0.30) \\ 
6448.844 & X-Ray$_\mathrm{swift}$ & [1.91(0.10)] & 1.77(0.15) \\ 
6450.361 & X-Ray$_\mathrm{swift}$ & [4.46(0.24)] & 1.72(0.14) \\ 
6451.052 & X-Ray$_\mathrm{swift}$ & [5.73(0.36)] & 1.72(0.13) \\ 
6454.146 & X-Ray$_\mathrm{swift}$ & [1.92(0.14)] & 1.79(0.15) \\ 
6457.990 & X-Ray$_\mathrm{swift}$ & [0.91(0.08)] & 1.62(0.19) \\ 
6458.323 & X-Ray$_\mathrm{swift}$ & [1.16(0.07)] & 1.67(0.25) \\ 
6459.059 & X-Ray$_\mathrm{swift}$ & [1.49(0.09)] & 1.76(0.25) \\ 
6460.260 & X-Ray$_\mathrm{swift}$ & [2.46(0.22)] & 1.70(0.16) \\ 
6461.859 & X-Ray$_\mathrm{swift}$ & [4.33(0.25)] & 1.78(0.20) \\ 
6462.394 & X-Ray$_\mathrm{swift}$ & [2.72(0.17)] & 1.63(0.12) \\ 
6463.069 & X-Ray$_\mathrm{swift}$ & [3.25(0.13)] & 1.84(0.14) \\ 
6413.896 & uvw2$_\mathrm{swift}$ & 14.48(0.03) & \nodata \\ 
6415.028 & uvw2$_\mathrm{swift}$ & 14.49(0.04) & \nodata \\ 
6415.559 & uvw2$_\mathrm{swift}$ & 14.53(0.04) & \nodata \\ 
6416.764 & uvw2$_\mathrm{swift}$ & 14.54(0.03) & \nodata \\ 
6417.509 & uvw2$_\mathrm{swift}$ & 14.49(0.03) & \nodata \\ 
6418.633 & uvw2$_\mathrm{swift}$ & 14.42(0.03) & \nodata \\ 
6419.505 & uvw2$_\mathrm{swift}$ & 14.31(0.04) & \nodata \\ 
6421.040 & uvw2$_\mathrm{swift}$ & 14.01(0.03) & \nodata \\ 
6421.841 & uvw2$_\mathrm{swift}$ & 13.90(0.03) & \nodata \\ 
6423.444 & uvw2$_\mathrm{swift}$ & 14.02(0.03) & \nodata \\ 
6424.252 & uvw2$_\mathrm{swift}$ & 13.80(0.03) & \nodata \\ 
6424.772 & uvw2$_\mathrm{swift}$ & 13.72(0.04) & \nodata \\ 
6426.311 & uvw2$_\mathrm{swift}$ & 13.70(0.03) & \nodata \\ 
6427.979 & uvw2$_\mathrm{swift}$ & 13.78(0.03) & \nodata \\ 
6431.603 & uvw2$_\mathrm{swift}$ & 13.72(0.04) & \nodata \\ 
6433.118 & uvw2$_\mathrm{swift}$ & 13.58(0.04) & \nodata \\ 
6434.252 & uvw2$_\mathrm{swift}$ & 13.55(0.03) & \nodata \\ 
6435.187 & uvw2$_\mathrm{swift}$ & 13.50(0.03) & \nodata \\ 
6436.073 & uvw2$_\mathrm{swift}$ & 13.52(0.03) & \nodata \\ 
6436.940 & uvw2$_\mathrm{swift}$ & 13.58(0.03) & \nodata \\ 
6437.928 & uvw2$_\mathrm{swift}$ & 13.65(0.03) & \nodata \\ 
6439.345 & uvw2$_\mathrm{swift}$ & 13.79(0.03) & \nodata \\ 
6440.080 & uvw2$_\mathrm{swift}$ & 13.76(0.03) & \nodata \\ 
6441.065 & uvw2$_\mathrm{swift}$ & 13.81(0.03) & \nodata \\ 
6442.015 & uvw2$_\mathrm{swift}$ & 13.85(0.03) & \nodata \\ 
6443.406 & uvw2$_\mathrm{swift}$ & 13.97(0.03) & \nodata \\ 
6444.340 & uvw2$_\mathrm{swift}$ & 14.09(0.03) & \nodata \\ 
6445.341 & uvw2$_\mathrm{swift}$ & 14.20(0.03) & \nodata \\ 
6446.021 & uvw2$_\mathrm{swift}$ & 14.39(0.03) & \nodata \\ 
6446.549 & uvw2$_\mathrm{swift}$ & 14.31(0.03) & \nodata \\ 
6447.541 & uvw2$_\mathrm{swift}$ & 14.40(0.03) & \nodata \\ 
6449.344 & uvw2$_\mathrm{swift}$ & 14.43(0.03) & \nodata \\ 
6450.742 & uvw2$_\mathrm{swift}$ & 14.44(0.04) & \nodata \\ 
6451.556 & uvw2$_\mathrm{swift}$ & 14.42(0.03) & \nodata \\ 
6454.616 & uvw2$_\mathrm{swift}$ & 14.54(0.04) & \nodata \\ 
6458.489 & uvw2$_\mathrm{swift}$ & 14.74(0.04) & \nodata \\ 
6458.823 & uvw2$_\mathrm{swift}$ & 14.77(0.04) & \nodata \\ 
6459.561 & uvw2$_\mathrm{swift}$ & 14.77(0.04) & \nodata \\ 
6460.760 & uvw2$_\mathrm{swift}$ & 14.75(0.04) & \nodata \\ 
6462.895 & uvw2$_\mathrm{swift}$ & 14.46(0.04) & \nodata \\ 
6463.570 & uvw2$_\mathrm{swift}$ & 14.52(0.03) & \nodata \\ 
6413.900 & uvm2$_\mathrm{swift}$ & 14.32(0.04) & \nodata \\ 
6415.031 & uvm2$_\mathrm{swift}$ & 14.31(0.04) & \nodata \\ 
6415.561 & uvm2$_\mathrm{swift}$ & 14.36(0.04) & \nodata \\ 
6416.769 & uvm2$_\mathrm{swift}$ & 14.35(0.04) & \nodata \\ 
6417.514 & uvm2$_\mathrm{swift}$ & 14.36(0.04) & \nodata \\ 
6418.638 & uvm2$_\mathrm{swift}$ & 14.29(0.04) & \nodata \\ 
6419.508 & uvm2$_\mathrm{swift}$ & 14.23(0.04) & \nodata \\ 
6421.044 & uvm2$_\mathrm{swift}$ & 13.95(0.04) & \nodata \\ 
6421.848 & uvm2$_\mathrm{swift}$ & 13.86(0.03) & \nodata \\ 
6423.451 & uvm2$_\mathrm{swift}$ & 13.97(0.03) & \nodata \\ 
6424.256 & uvm2$_\mathrm{swift}$ & 13.76(0.04) & \nodata \\ 
6424.774 & uvm2$_\mathrm{swift}$ & 13.76(0.04) & \nodata \\ 
6426.316 & uvm2$_\mathrm{swift}$ & 13.67(0.03) & \nodata \\ 
6427.984 & uvm2$_\mathrm{swift}$ & 13.71(0.04) & \nodata \\ 
6431.605 & uvm2$_\mathrm{swift}$ & 13.72(0.04) & \nodata \\ 
6433.120 & uvm2$_\mathrm{swift}$ & 13.57(0.04) & \nodata \\ 
6434.254 & uvm2$_\mathrm{swift}$ & 13.52(0.04) & \nodata \\ 
6435.189 & uvm2$_\mathrm{swift}$ & 13.42(0.04) & \nodata \\ 
6436.078 & uvm2$_\mathrm{swift}$ & 13.53(0.03) & \nodata \\ 
6436.944 & uvm2$_\mathrm{swift}$ & 13.56(0.03) & \nodata \\ 
6437.932 & uvm2$_\mathrm{swift}$ & 13.59(0.04) & \nodata \\ 
6439.349 & uvm2$_\mathrm{swift}$ & 13.73(0.04) & \nodata \\ 
6440.084 & uvm2$_\mathrm{swift}$ & 13.71(0.04) & \nodata \\ 
6441.068 & uvm2$_\mathrm{swift}$ & 13.76(0.04) & \nodata \\ 
6442.020 & uvm2$_\mathrm{swift}$ & 13.79(0.04) & \nodata \\ 
6443.411 & uvm2$_\mathrm{swift}$ & 13.86(0.03) & \nodata \\ 
6444.344 & uvm2$_\mathrm{swift}$ & 13.97(0.04) & \nodata \\ 
6445.345 & uvm2$_\mathrm{swift}$ & 14.06(0.04) & \nodata \\ 
6446.026 & uvm2$_\mathrm{swift}$ & 14.22(0.04) & \nodata \\ 
6446.553 & uvm2$_\mathrm{swift}$ & 14.16(0.04) & \nodata \\ 
6447.545 & uvm2$_\mathrm{swift}$ & 14.23(0.04) & \nodata \\ 
6449.348 & uvm2$_\mathrm{swift}$ & 14.34(0.04) & \nodata \\ 
6450.745 & uvm2$_\mathrm{swift}$ & 14.27(0.04) & \nodata \\ 
6454.618 & uvm2$_\mathrm{swift}$ & 14.40(0.05) & \nodata \\ 
6458.493 & uvm2$_\mathrm{swift}$ & 14.57(0.04) & \nodata \\ 
6458.828 & uvm2$_\mathrm{swift}$ & 14.60(0.04) & \nodata \\ 
6459.565 & uvm2$_\mathrm{swift}$ & 14.58(0.04) & \nodata \\ 
6460.764 & uvm2$_\mathrm{swift}$ & 14.61(0.04) & \nodata \\ 
6462.899 & uvm2$_\mathrm{swift}$ & 14.39(0.04) & \nodata \\ 
6463.575 & uvm2$_\mathrm{swift}$ & 14.40(0.04) & \nodata \\ 
6413.891 & uvw1$_\mathrm{swift}$ & 14.17(0.04) & \nodata \\ 
6415.025 & uvw1$_\mathrm{swift}$ & 14.14(0.04) & \nodata \\ 
6415.555 & uvw1$_\mathrm{swift}$ & 14.12(0.04) & \nodata \\ 
6416.757 & uvw1$_\mathrm{swift}$ & 14.16(0.04) & \nodata \\ 
6417.502 & uvw1$_\mathrm{swift}$ & 14.20(0.04) & \nodata \\ 
6418.627 & uvw1$_\mathrm{swift}$ & 14.15(0.04) & \nodata \\ 
6419.502 & uvw1$_\mathrm{swift}$ & 14.12(0.04) & \nodata \\ 
6421.034 & uvw1$_\mathrm{swift}$ & 13.92(0.04) & \nodata \\ 
6421.833 & uvw1$_\mathrm{swift}$ & 13.79(0.03) & \nodata \\ 
6423.436 & uvw1$_\mathrm{swift}$ & 13.83(0.03) & \nodata \\ 
6424.246 & uvw1$_\mathrm{swift}$ & 13.66(0.03) & \nodata \\ 
6424.770 & uvw1$_\mathrm{swift}$ & 13.70(0.04) & \nodata \\ 
6426.305 & uvw1$_\mathrm{swift}$ & 13.63(0.03) & \nodata \\ 
6427.974 & uvw1$_\mathrm{swift}$ & 13.63(0.03) & \nodata \\ 
6431.600 & uvw1$_\mathrm{swift}$ & 13.62(0.04) & \nodata \\ 
6433.115 & uvw1$_\mathrm{swift}$ & 13.49(0.04) & \nodata \\ 
6434.250 & uvw1$_\mathrm{swift}$ & 13.63(0.04) & \nodata \\ 
6435.185 & uvw1$_\mathrm{swift}$ & 13.40(0.04) & \nodata \\ 
6436.068 & uvw1$_\mathrm{swift}$ & 13.50(0.03) & \nodata \\ 
6436.935 & uvw1$_\mathrm{swift}$ & 13.53(0.03) & \nodata \\ 
6437.923 & uvw1$_\mathrm{swift}$ & 13.52(0.03) & \nodata \\ 
6439.340 & uvw1$_\mathrm{swift}$ & 13.60(0.03) & \nodata \\ 
6440.075 & uvw1$_\mathrm{swift}$ & 13.66(0.03) & \nodata \\ 
6441.061 & uvw1$_\mathrm{swift}$ & 13.67(0.04) & \nodata \\ 
6442.010 & uvw1$_\mathrm{swift}$ & 13.65(0.03) & \nodata \\ 
6443.399 & uvw1$_\mathrm{swift}$ & 13.72(0.03) & \nodata \\ 
6444.335 & uvw1$_\mathrm{swift}$ & 13.80(0.04) & \nodata \\ 
6445.336 & uvw1$_\mathrm{swift}$ & 13.87(0.04) & \nodata \\ 
6446.016 & uvw1$_\mathrm{swift}$ & 13.99(0.04) & \nodata \\ 
6446.544 & uvw1$_\mathrm{swift}$ & 14.00(0.04) & \nodata \\ 
6447.536 & uvw1$_\mathrm{swift}$ & 14.03(0.04) & \nodata \\ 
6449.339 & uvw1$_\mathrm{swift}$ & 14.08(0.04) & \nodata \\ 
6450.740 & uvw1$_\mathrm{swift}$ & 14.12(0.04) & \nodata \\ 
6451.550 & uvw1$_\mathrm{swift}$ & 14.08(0.04) & \nodata \\ 
6454.614 & uvw1$_\mathrm{swift}$ & 14.12(0.04) & \nodata \\ 
6458.485 & uvw1$_\mathrm{swift}$ & 14.35(0.04) & \nodata \\ 
6458.818 & uvw1$_\mathrm{swift}$ & 14.38(0.04) & \nodata \\ 
6459.555 & uvw1$_\mathrm{swift}$ & 14.35(0.04) & \nodata \\ 
6460.754 & uvw1$_\mathrm{swift}$ & 14.31(0.04) & \nodata \\ 
6462.890 & uvw1$_\mathrm{swift}$ & 14.17(0.04) & \nodata \\ 
6463.566 & uvw1$_\mathrm{swift}$ & 14.22(0.04) & \nodata \\ 
6413.892 & $U_\mathrm{swift}$ & 14.22(0.03) & \nodata \\ 
6415.026 & $U_\mathrm{swift}$ & 14.30(0.03) & \nodata \\ 
6415.556 & $U_\mathrm{swift}$ & 14.24(0.03) & \nodata \\ 
6416.759 & $U_\mathrm{swift}$ & 14.27(0.03) & \nodata \\ 
6417.504 & $U_\mathrm{swift}$ & 14.24(0.03) & \nodata \\ 
6418.629 & $U_\mathrm{swift}$ & 14.20(0.03) & \nodata \\ 
6419.503 & $U_\mathrm{swift}$ & 14.23(0.03) & \nodata \\ 
6421.036 & $U_\mathrm{swift}$ & 14.03(0.03) & \nodata \\ 
6421.835 & $U_\mathrm{swift}$ & 13.91(0.03) & \nodata \\ 
6423.438 & $U_\mathrm{swift}$ & 13.88(0.03) & \nodata \\ 
6424.248 & $U_\mathrm{swift}$ & 13.79(0.03) & \nodata \\ 
6424.771 & $U_\mathrm{swift}$ & 13.73(0.03) & \nodata \\ 
6426.307 & $U_\mathrm{swift}$ & 13.73(0.03) & \nodata \\ 
6427.976 & $U_\mathrm{swift}$ & 13.74(0.03) & \nodata \\ 
6431.601 & $U_\mathrm{swift}$ & 13.72(0.03) & \nodata \\ 
6433.116 & $U_\mathrm{swift}$ & 13.66(0.03) & \nodata \\ 
6434.250 & $U_\mathrm{swift}$ & 13.65(0.03) & \nodata \\ 
6435.186 & $U_\mathrm{swift}$ & 13.59(0.03) & \nodata \\ 
6436.070 & $U_\mathrm{swift}$ & 13.60(0.03) & \nodata \\ 
6436.937 & $U_\mathrm{swift}$ & 13.64(0.03) & \nodata \\ 
6437.925 & $U_\mathrm{swift}$ & 13.62(0.03) & \nodata \\ 
6439.341 & $U_\mathrm{swift}$ & 13.69(0.03) & \nodata \\ 
6440.076 & $U_\mathrm{swift}$ & 13.68(0.03) & \nodata \\ 
6441.062 & $U_\mathrm{swift}$ & 13.69(0.03) & \nodata \\ 
6442.012 & $U_\mathrm{swift}$ & 13.76(0.03) & \nodata \\ 
6443.401 & $U_\mathrm{swift}$ & 13.79(0.03) & \nodata \\ 
6444.336 & $U_\mathrm{swift}$ & 13.83(0.03) & \nodata \\ 
6445.338 & $U_\mathrm{swift}$ & 13.97(0.03) & \nodata \\ 
6446.018 & $U_\mathrm{swift}$ & 14.10(0.03) & \nodata \\ 
6446.546 & $U_\mathrm{swift}$ & 14.01(0.03) & \nodata \\ 
6447.538 & $U_\mathrm{swift}$ & 14.14(0.03) & \nodata \\ 
6449.341 & $U_\mathrm{swift}$ & 14.19(0.03) & \nodata \\ 
6450.741 & $U_\mathrm{swift}$ & 14.19(0.04) & \nodata \\ 
6451.552 & $U_\mathrm{swift}$ & 14.17(0.03) & \nodata \\ 
6454.614 & $U_\mathrm{swift}$ & 14.21(0.04) & \nodata \\ 
6458.486 & $U_\mathrm{swift}$ & 14.38(0.03) & \nodata \\ 
6458.820 & $U_\mathrm{swift}$ & 14.41(0.03) & \nodata \\ 
6459.557 & $U_\mathrm{swift}$ & 14.42(0.03) & \nodata \\ 
6460.756 & $U_\mathrm{swift}$ & 14.40(0.03) & \nodata \\ 
6462.891 & $U_\mathrm{swift}$ & 14.22(0.03) & \nodata \\ 
6463.567 & $U_\mathrm{swift}$ & 14.28(0.03) & \nodata \\ 
6433.483 & $u$ & 14.69(0.03) & \nodata \\ 
6434.544 & $u$ & 14.69(0.02) & \nodata \\ 
6435.509 & $u$ & 14.66(0.02) & \nodata \\ 
6436.489 & $u$ & 14.64(0.02) & \nodata \\ 
6437.474 & $u$ & 14.64(0.02) & \nodata \\ 
6438.484 & $u$ & 14.68(0.02) & \nodata \\ 
6406.570 & $B$ & 14.92(0.03) & \nodata \\ 
6406.572 & $B$ & 14.92(0.03) & \nodata \\ 
6407.503 & $B$ & 14.88(0.04) & \nodata \\ 
6408.471 & $B$ & 14.87(0.03) & \nodata \\ 
6417.477 & $B$ & 15.02(0.04) & \nodata \\ 
6433.486 & $B$ & 14.65(0.03) & \nodata \\ 
6434.466 & $B$ & 14.61(0.02) & \nodata \\ 
6434.468 & $B$ & 14.61(0.02) & \nodata \\ 
6434.551 & $B$ & 14.61(0.02) & \nodata \\ 
6435.466 & $B$ & 14.59(0.02) & \nodata \\ 
6435.468 & $B$ & 14.60(0.02) & \nodata \\ 
6435.496 & $B$ & 14.58(0.03) & \nodata \\ 
6436.474 & $B$ & 14.59(0.03) & \nodata \\ 
6437.478 & $B$ & 14.60(0.03) & \nodata \\ 
6438.491 & $B$ & 14.64(0.03) & \nodata \\ 
6439.479 & $B$ & 14.67(0.02) & \nodata \\ 
6439.481 & $B$ & 14.67(0.03) & \nodata \\ 
6442.479 & $B$ & 14.73(0.03) & \nodata \\ 
6442.481 & $B$ & 14.72(0.03) & \nodata \\ 
6413.893 & $B_\mathrm{swift}$ & 15.08(0.03) & \nodata \\ 
6415.027 & $B_\mathrm{swift}$ & 15.12(0.03) & \nodata \\ 
6415.557 & $B_\mathrm{swift}$ & 15.01(0.03) & \nodata \\ 
6416.761 & $B_\mathrm{swift}$ & 15.06(0.03) & \nodata \\ 
6417.506 & $B_\mathrm{swift}$ & 15.12(0.03) & \nodata \\ 
6418.630 & $B_\mathrm{swift}$ & 15.10(0.03) & \nodata \\ 
6419.504 & $B_\mathrm{swift}$ & 15.02(0.03) & \nodata \\ 
6421.037 & $B_\mathrm{swift}$ & 14.95(0.03) & \nodata \\ 
6421.837 & $B_\mathrm{swift}$ & 14.86(0.03) & \nodata \\ 
6423.440 & $B_\mathrm{swift}$ & 14.86(0.03) & \nodata \\ 
6424.249 & $B_\mathrm{swift}$ & 14.79(0.03) & \nodata \\ 
6424.771 & $B_\mathrm{swift}$ & 14.76(0.04) & \nodata \\ 
6426.308 & $B_\mathrm{swift}$ & 14.79(0.03) & \nodata \\ 
6427.977 & $B_\mathrm{swift}$ & 14.76(0.03) & \nodata \\ 
6431.602 & $B_\mathrm{swift}$ & 14.81(0.03) & \nodata \\ 
6433.117 & $B_\mathrm{swift}$ & 14.73(0.04) & \nodata \\ 
6434.251 & $B_\mathrm{swift}$ & 14.65(0.03) & \nodata \\ 
6435.186 & $B_\mathrm{swift}$ & 14.62(0.03) & \nodata \\ 
6436.071 & $B_\mathrm{swift}$ & 14.71(0.03) & \nodata \\ 
6436.938 & $B_\mathrm{swift}$ & 14.70(0.03) & \nodata \\ 
6437.926 & $B_\mathrm{swift}$ & 14.70(0.03) & \nodata \\ 
6439.342 & $B_\mathrm{swift}$ & 14.77(0.03) & \nodata \\ 
6440.077 & $B_\mathrm{swift}$ & 14.76(0.03) & \nodata \\ 
6441.063 & $B_\mathrm{swift}$ & 14.76(0.03) & \nodata \\ 
6442.013 & $B_\mathrm{swift}$ & 14.78(0.03) & \nodata \\ 
6443.402 & $B_\mathrm{swift}$ & 14.83(0.03) & \nodata \\ 
6444.337 & $B_\mathrm{swift}$ & 14.86(0.03) & \nodata \\ 
6445.339 & $B_\mathrm{swift}$ & 14.94(0.03) & \nodata \\ 
6446.019 & $B_\mathrm{swift}$ & 14.97(0.03) & \nodata \\ 
6446.547 & $B_\mathrm{swift}$ & 14.97(0.03) & \nodata \\ 
6447.539 & $B_\mathrm{swift}$ & 14.96(0.03) & \nodata \\ 
6449.342 & $B_\mathrm{swift}$ & 15.06(0.03) & \nodata \\ 
6450.741 & $B_\mathrm{swift}$ & 14.98(0.04) & \nodata \\ 
6451.553 & $B_\mathrm{swift}$ & 15.01(0.03) & \nodata \\ 
6454.615 & $B_\mathrm{swift}$ & 15.03(0.04) & \nodata \\ 
6458.487 & $B_\mathrm{swift}$ & 15.11(0.03) & \nodata \\ 
6458.821 & $B_\mathrm{swift}$ & 15.13(0.03) & \nodata \\ 
6459.558 & $B_\mathrm{swift}$ & 15.12(0.03) & \nodata \\ 
6460.757 & $B_\mathrm{swift}$ & 15.13(0.03) & \nodata \\ 
6462.892 & $B_\mathrm{swift}$ & 15.01(0.03) & \nodata \\ 
6463.568 & $B_\mathrm{swift}$ & 15.07(0.03) & \nodata \\ 
6406.645 & $g$ & 14.55(0.03) & \nodata \\ 
6409.632 & $g$ & 14.60(0.03) & \nodata \\ 
6409.632 & $g$ & 14.60(0.03) & \nodata \\ 
6409.632 & $g$ & 14.60(0.03) & \nodata \\ 
6411.628 & $g$ & 14.66(0.03) & \nodata \\ 
6411.629 & $g$ & 14.65(0.03) & \nodata \\ 
6411.629 & $g$ & 14.66(0.03) & \nodata \\ 
6412.629 & $g$ & 14.69(0.03) & \nodata \\ 
6412.629 & $g$ & 14.69(0.03) & \nodata \\ 
6412.630 & $g$ & 14.68(0.03) & \nodata \\ 
6413.628 & $g$ & 14.71(0.02) & \nodata \\ 
6413.629 & $g$ & 14.70(0.02) & \nodata \\ 
6413.630 & $g$ & 14.70(0.03) & \nodata \\ 
6414.466 & $g$ & 14.63(0.04) & \nodata \\ 
6424.456 & $g$ & 14.40(0.04) & \nodata \\ 
6433.477 & $g$ & 14.34(0.03) & \nodata \\ 
6434.540 & $g$ & 14.31(0.03) & \nodata \\ 
6435.501 & $g$ & 14.27(0.03) & \nodata \\ 
6436.478 & $g$ & 14.29(0.03) & \nodata \\ 
6437.464 & $g$ & 14.30(0.03) & \nodata \\ 
6438.472 & $g$ & 14.32(0.03) & \nodata \\ 
6406.575 & $V$ & 14.32(0.03) & \nodata \\ 
6406.577 & $V$ & 14.31(0.03) & \nodata \\ 
6407.501 & $V$ & 14.30(0.04) & \nodata \\ 
6408.468 & $V$ & 14.31(0.03) & \nodata \\ 
6417.479 & $V$ & 14.38(0.04) & \nodata \\ 
6433.484 & $V$ & 14.15(0.03) & \nodata \\ 
6434.469 & $V$ & 14.12(0.02) & \nodata \\ 
6434.471 & $V$ & 14.12(0.02) & \nodata \\ 
6434.546 & $V$ & 14.12(0.03) & \nodata \\ 
6435.470 & $V$ & 14.12(0.02) & \nodata \\ 
6435.471 & $V$ & 14.12(0.02) & \nodata \\ 
6435.498 & $V$ & 14.11(0.03) & \nodata \\ 
6436.472 & $V$ & 14.11(0.03) & \nodata \\ 
6437.476 & $V$ & 14.12(0.03) & \nodata \\ 
6438.469 & $V$ & 14.14(0.02) & \nodata \\ 
6438.487 & $V$ & 14.13(0.03) & \nodata \\ 
6439.483 & $V$ & 14.15(0.03) & \nodata \\ 
6439.484 & $V$ & 14.14(0.03) & \nodata \\ 
6442.483 & $V$ & 14.17(0.03) & \nodata \\ 
6442.484 & $V$ & 14.18(0.03) & \nodata \\ 
6413.898 & $V_\mathrm{swift}$ & 14.54(0.03) & \nodata \\ 
6415.030 & $V_\mathrm{swift}$ & 14.52(0.04) & \nodata \\ 
6415.560 & $V_\mathrm{swift}$ & 14.52(0.04) & \nodata \\ 
6416.767 & $V_\mathrm{swift}$ & 14.54(0.03) & \nodata \\ 
6417.513 & $V_\mathrm{swift}$ & 14.52(0.03) & \nodata \\ 
6418.636 & $V_\mathrm{swift}$ & 14.54(0.03) & \nodata \\ 
6419.507 & $V_\mathrm{swift}$ & 14.47(0.04) & \nodata \\ 
6421.042 & $V_\mathrm{swift}$ & 14.51(0.03) & \nodata \\ 
6421.845 & $V_\mathrm{swift}$ & 14.43(0.02) & \nodata \\ 
6423.448 & $V_\mathrm{swift}$ & 14.39(0.02) & \nodata \\ 
6424.254 & $V_\mathrm{swift}$ & 14.35(0.03) & \nodata \\ 
6424.773 & $V_\mathrm{swift}$ & 14.36(0.04) & \nodata \\ 
6426.314 & $V_\mathrm{swift}$ & 14.35(0.03) & \nodata \\ 
6427.982 & $V_\mathrm{swift}$ & 14.34(0.03) & \nodata \\ 
6431.604 & $V_\mathrm{swift}$ & 14.30(0.04) & \nodata \\ 
6433.119 & $V_\mathrm{swift}$ & 14.28(0.04) & \nodata \\ 
6434.253 & $V_\mathrm{swift}$ & 14.31(0.04) & \nodata \\ 
6435.188 & $V_\mathrm{swift}$ & 14.30(0.04) & \nodata \\ 
6436.076 & $V_\mathrm{swift}$ & 14.36(0.03) & \nodata \\ 
6436.942 & $V_\mathrm{swift}$ & 14.32(0.03) & \nodata \\ 
6437.930 & $V_\mathrm{swift}$ & 14.24(0.03) & \nodata \\ 
6439.347 & $V_\mathrm{swift}$ & 14.38(0.03) & \nodata \\ 
6440.082 & $V_\mathrm{swift}$ & 14.37(0.03) & \nodata \\ 
6441.067 & $V_\mathrm{swift}$ & 14.30(0.03) & \nodata \\ 
6442.018 & $V_\mathrm{swift}$ & 14.36(0.03) & \nodata \\ 
6443.409 & $V_\mathrm{swift}$ & 14.32(0.02) & \nodata \\ 
6444.342 & $V_\mathrm{swift}$ & 14.45(0.03) & \nodata \\ 
6445.343 & $V_\mathrm{swift}$ & 14.40(0.03) & \nodata \\ 
6446.024 & $V_\mathrm{swift}$ & 14.52(0.03) & \nodata \\ 
6446.551 & $V_\mathrm{swift}$ & 14.43(0.03) & \nodata \\ 
6447.543 & $V_\mathrm{swift}$ & 14.47(0.03) & \nodata \\ 
6449.347 & $V_\mathrm{swift}$ & 14.51(0.03) & \nodata \\ 
6450.744 & $V_\mathrm{swift}$ & 14.47(0.04) & \nodata \\ 
6451.558 & $V_\mathrm{swift}$ & 14.54(0.05) & \nodata \\ 
6454.617 & $V_\mathrm{swift}$ & 14.48(0.04) & \nodata \\ 
6458.492 & $V_\mathrm{swift}$ & 14.52(0.03) & \nodata \\ 
6458.826 & $V_\mathrm{swift}$ & 14.57(0.03) & \nodata \\ 
6459.563 & $V_\mathrm{swift}$ & 14.53(0.03) & \nodata \\ 
6460.762 & $V_\mathrm{swift}$ & 14.56(0.03) & \nodata \\ 
6462.897 & $V_\mathrm{swift}$ & 14.51(0.03) & \nodata \\ 
6463.573 & $V_\mathrm{swift}$ & 14.46(0.03) & \nodata \\ 
6406.683 & $r$ & 13.88(0.02) & \nodata \\ 
6406.686 & $r$ & 13.88(0.02) & \nodata \\ 
6406.688 & $r$ & 13.87(0.02) & \nodata \\ 
6407.498 & $r$ & 13.88(0.03) & \nodata \\ 
6408.476 & $r$ & 13.87(0.03) & \nodata \\ 
6409.634 & $r$ & 13.97(0.02) & \nodata \\ 
6409.635 & $r$ & 13.97(0.02) & \nodata \\ 
6409.635 & $r$ & 13.97(0.02) & \nodata \\ 
6411.630 & $r$ & 13.98(0.03) & \nodata \\ 
6411.631 & $r$ & 13.98(0.02) & \nodata \\ 
6411.631 & $r$ & 13.98(0.03) & \nodata \\ 
6412.631 & $r$ & 13.99(0.03) & \nodata \\ 
6412.631 & $r$ & 13.99(0.03) & \nodata \\ 
6412.631 & $r$ & 13.99(0.03) & \nodata \\ 
6413.631 & $r$ & 14.01(0.02) & \nodata \\ 
6413.632 & $r$ & 14.00(0.02) & \nodata \\ 
6413.632 & $r$ & 14.00(0.02) & \nodata \\ 
6414.467 & $r$ & 13.93(0.03) & \nodata \\ 
6417.481 & $r$ & 13.94(0.03) & \nodata \\ 
6424.454 & $r$ & 13.80(0.03) & \nodata \\ 
6434.537 & $r$ & 13.73(0.03) & \nodata \\ 
6433.479 & $r$ & 13.75(0.02) & \nodata \\ 
6435.503 & $r$ & 13.71(0.03) & \nodata \\ 
6436.481 & $r$ & 13.71(0.03) & \nodata \\ 
6437.467 & $r$ & 13.72(0.03) & \nodata \\ 
6438.476 & $r$ & 13.72(0.03) & \nodata \\ 
6434.472 & $R$ & 13.58(0.02) & \nodata \\ 
6434.474 & $R$ & 13.58(0.02) & \nodata \\ 
6435.472 & $R$ & 13.56(0.02) & \nodata \\ 
6435.474 & $R$ & 13.57(0.02) & \nodata \\ 
6438.473 & $R$ & 13.56(0.02) & \nodata \\ 
6439.486 & $R$ & 13.58(0.02) & \nodata \\ 
6439.487 & $R$ & 13.57(0.02) & \nodata \\ 
6442.485 & $R$ & 13.60(0.03) & \nodata \\ 
6442.487 & $R$ & 13.59(0.03) & \nodata \\ 
6407.499 & $i$ & 13.69(0.03) & \nodata \\ 
6408.474 & $i$ & 13.68(0.03) & \nodata \\ 
6409.636 & $i$ & 13.77(0.02) & \nodata \\ 
6409.637 & $i$ & 13.77(0.02) & \nodata \\ 
6409.637 & $i$ & 13.77(0.02) & \nodata \\ 
6411.633 & $i$ & 13.78(0.02) & \nodata \\ 
6411.634 & $i$ & 13.78(0.02) & \nodata \\ 
6411.634 & $i$ & 13.78(0.02) & \nodata \\ 
6412.633 & $i$ & 13.80(0.03) & \nodata \\ 
6412.633 & $i$ & 13.80(0.03) & \nodata \\ 
6412.634 & $i$ & 13.80(0.03) & \nodata \\ 
6413.634 & $i$ & 13.79(0.02) & \nodata \\ 
6413.634 & $i$ & 13.79(0.02) & \nodata \\ 
6413.635 & $i$ & 13.79(0.02) & \nodata \\ 
6414.469 & $i$ & 13.74(0.03) & \nodata \\ 
6417.482 & $i$ & 13.74(0.03) & \nodata \\ 
6424.453 & $i$ & 13.62(0.03) & \nodata \\ 
6433.480 & $i$ & 13.59(0.02) & \nodata \\ 
6434.534 & $i$ & 13.57(0.02) & \nodata \\ 
6435.505 & $i$ & 13.56(0.03) & \nodata \\ 
6436.483 & $i$ & 13.55(0.03) & \nodata \\ 
6437.469 & $i$ & 13.55(0.03) & \nodata \\ 
6438.479 & $i$ & 13.55(0.03) & \nodata \\ 
6434.475 & $I$ & 13.13(0.02) & \nodata \\ 
6434.476 & $I$ & 13.13(0.02) & \nodata \\ 
6435.475 & $I$ & 13.12(0.02) & \nodata \\ 
6435.476 & $I$ & 13.11(0.02) & \nodata \\ 
6438.476 & $I$ & 13.11(0.02) & \nodata \\ 
6439.488 & $I$ & 13.12(0.02) & \nodata \\ 
6439.489 & $I$ & 13.11(0.02) & \nodata \\ 
6442.488 & $I$ & 13.12(0.03) & \nodata \\ 
6442.489 & $I$ & 13.12(0.03) & \nodata \\ 
6408.787 & $Z$ & 12.96(0.01) & \nodata \\ 
6409.733 & $Z$ & 12.96(0.01) & \nodata \\ 
6410.737 & $Z$ & 12.96(0.01) & \nodata \\ 
6411.733 & $Z$ & 12.94(0.01) & \nodata \\ 
6412.735 & $Z$ & 12.96(0.01) & \nodata \\ 
6413.729 & $Z$ & 12.97(0.01) & \nodata \\ 
6414.729 & $Z$ & 12.97(0.01) & \nodata \\ 
6415.729 & $Z$ & 12.98(0.01) & \nodata \\ 
6416.728 & $Z$ & 12.98(0.01) & \nodata \\ 
6417.727 & $Z$ & 12.98(0.01) & \nodata \\ 
6419.732 & $Z$ & 12.98(0.01) & \nodata \\ 
6420.736 & $Z$ & 12.96(0.01) & \nodata \\ 
6422.736 & $Z$ & 12.93(0.01) & \nodata \\ 
6424.739 & $Z$ & 12.90(0.01) & \nodata \\ 
6426.780 & $Z$ & 12.86(0.01) & \nodata \\ 
6430.733 & $Z$ & 12.86(0.01) & \nodata \\ 
6433.738 & $Z$ & 12.86(0.01) & \nodata \\ 
6435.742 & $Z$ & 12.84(0.01) & \nodata \\ 
6437.745 & $Z$ & 12.83(0.01) & \nodata \\ 
6439.742 & $Z$ & 12.82(0.01) & \nodata \\ 
6442.746 & $Z$ & 12.86(0.01) & \nodata \\ 
6408.785 & $Y$ & 12.71(0.01) & \nodata \\ 
6409.731 & $Y$ & 12.71(0.01) & \nodata \\ 
6410.735 & $Y$ & 12.71(0.01) & \nodata \\ 
6411.730 & $Y$ & 12.71(0.01) & \nodata \\ 
6412.732 & $Y$ & 12.72(0.01) & \nodata \\ 
6413.726 & $Y$ & 12.73(0.01) & \nodata \\ 
6414.727 & $Y$ & 12.72(0.01) & \nodata \\ 
6415.727 & $Y$ & 12.74(0.01) & \nodata \\ 
6416.726 & $Y$ & 12.73(0.01) & \nodata \\ 
6417.725 & $Y$ & 12.73(0.01) & \nodata \\ 
6419.729 & $Y$ & 12.72(0.01) & \nodata \\ 
6420.734 & $Y$ & 12.71(0.01) & \nodata \\ 
6422.734 & $Y$ & 12.68(0.01) & \nodata \\ 
6424.737 & $Y$ & 12.66(0.01) & \nodata \\ 
6426.778 & $Y$ & 12.64(0.01) & \nodata \\ 
6430.731 & $Y$ & 12.64(0.01) & \nodata \\ 
6433.736 & $Y$ & 12.63(0.01) & \nodata \\ 
6435.740 & $Y$ & 12.61(0.01) & \nodata \\ 
6437.742 & $Y$ & 12.58(0.01) & \nodata \\ 
6439.740 & $Y$ & 12.59(0.01) & \nodata \\ 
6442.743 & $Y$ & 12.62(0.01) & \nodata \\ 
6408.782 & $J$ & 12.18(0.01) & \nodata \\ 
6409.729 & $J$ & 12.18(0.01) & \nodata \\ 
6410.732 & $J$ & 12.17(0.01) & \nodata \\ 
6411.728 & $J$ & 12.18(0.01) & \nodata \\ 
6412.730 & $J$ & 12.18(0.02) & \nodata \\ 
6413.724 & $J$ & 12.18(0.02) & \nodata \\ 
6414.725 & $J$ & 12.18(0.02) & \nodata \\ 
6415.725 & $J$ & 12.19(0.02) & \nodata \\ 
6416.723 & $J$ & 12.17(0.01) & \nodata \\ 
6417.723 & $J$ & 12.18(0.01) & \nodata \\ 
6419.727 & $J$ & 12.18(0.01) & \nodata \\ 
6420.732 & $J$ & 12.17(0.01) & \nodata \\ 
6422.732 & $J$ & 12.14(0.02) & \nodata \\ 
6424.735 & $J$ & 12.13(0.02) & \nodata \\ 
6426.776 & $J$ & 12.09(0.01) & \nodata \\ 
6430.729 & $J$ & 12.10(0.01) & \nodata \\ 
6433.734 & $J$ & 12.10(0.01) & \nodata \\ 
6435.738 & $J$ & 12.08(0.01) & \nodata \\ 
6437.740 & $J$ & 12.07(0.01) & \nodata \\ 
6439.737 & $J$ & 12.03(0.02) & \nodata \\ 
6442.741 & $J$ & 12.06(0.01) & \nodata \\ 
6444.735 & $J$ & 12.04(0.02) & \nodata \\ 
6408.780 & $H$ & 11.51(0.03) & \nodata \\ 
6409.726 & $H$ & 11.52(0.02) & \nodata \\ 
6410.730 & $H$ & 11.51(0.02) & \nodata \\ 
6411.726 & $H$ & 11.51(0.02) & \nodata \\ 
6412.728 & $H$ & 11.50(0.02) & \nodata \\ 
6413.722 & $H$ & 11.49(0.02) & \nodata \\ 
6414.722 & $H$ & 11.50(0.02) & \nodata \\ 
6415.723 & $H$ & 11.50(0.03) & \nodata \\ 
6416.721 & $H$ & 11.49(0.02) & \nodata \\ 
6417.721 & $H$ & 11.50(0.02) & \nodata \\ 
6419.725 & $H$ & 11.49(0.02) & \nodata \\ 
6420.729 & $H$ & 11.48(0.02) & \nodata \\ 
6422.730 & $H$ & 11.46(0.02) & \nodata \\ 
6424.733 & $H$ & 11.45(0.03) & \nodata \\ 
6426.763 & $H$ & 11.41(0.02) & \nodata \\ 
6430.727 & $H$ & 11.42(0.02) & \nodata \\ 
6433.731 & $H$ & 11.41(0.02) & \nodata \\ 
6435.735 & $H$ & 11.41(0.02) & \nodata \\ 
6437.738 & $H$ & 11.38(0.02) & \nodata \\ 
6439.735 & $H$ & 11.36(0.02) & \nodata \\ 
6442.734 & $H$ & 11.37(0.02) & \nodata \\ 
6442.739 & $H$ & 11.36(0.03) & \nodata \\ 
6444.733 & $H$ & 11.32(0.03) & \nodata \\ 
6408.777 & $K$ & 11.05(0.03) & \nodata \\ 
6409.724 & $K$ & 11.03(0.03) & \nodata \\ 
6410.728 & $K$ & 11.02(0.03) & \nodata \\ 
6411.723 & $K$ & 11.01(0.03) & \nodata \\ 
6412.726 & $K$ & 11.01(0.03) & \nodata \\ 
6413.720 & $K$ & 11.01(0.03) & \nodata \\ 
6414.720 & $K$ & 11.01(0.03) & \nodata \\ 
6415.721 & $K$ & 11.00(0.03) & \nodata \\ 
6416.719 & $K$ & 11.00(0.03) & \nodata \\ 
6417.719 & $K$ & 10.99(0.02) & \nodata \\ 
6419.723 & $K$ & 11.00(0.03) & \nodata \\ 
6420.727 & $K$ & 10.93(0.03) & \nodata \\ 
6422.728 & $K$ & 10.96(0.03) & \nodata \\ 
6424.731 & $K$ & 10.95(0.03) & \nodata \\ 
6426.759 & $K$ & 10.92(0.03) & \nodata \\ 
6430.725 & $K$ & 10.90(0.03) & \nodata \\ 
6433.729 & $K$ & 10.89(0.03) & \nodata \\ 
6435.733 & $K$ & 10.87(0.03) & \nodata \\ 
6437.736 & $K$ & 10.84(0.03) & \nodata \\ 
6439.732 & $K$ & 10.82(0.02) & \nodata \\ 
6442.731 & $K$ & 10.82(0.03) & \nodata \\ 
6444.732 & $K$ & 10.74(0.03) & \nodata \\ 
\enddata \tablecomments{\swift, $U$, $B$, $V$, $R$, $I$, $Z$, $Y$, $J$, $H$, and $K\--\textrm{band}$ photometry are calibrated in the Vega magnitude system. $u'$, $g'$, $r'$, and $i'\--\textrm{band}$ photometry are calibrated in the AB magnitude system.  X-Ray fluxes (0.3$\--$10 keV) are in units of $10^{-11}$ ergs/cm$^{2}$/s.} 
\label{tab:phot} 
\end{deluxetable} 

